A Network Arena for Benchmarking AI Agents on Network Troubleshooting

Agentic systems, powered by Large Language Models (LLMs), assist network engineers with network configuration synthesis and network troubleshooting tasks. For network troubleshooting, progress is hindered by the absence of standardized and accessible benchmarks for evaluating LLM agents in dynamic network settings at low operational effort. We present NIKA, the largest public benchmark to date for LLM-driven network incident diagnosis and troubleshooting. NIKA targets both domain experts and especially AI researchers alike, providing zero-effort replay of real-world network scenarios, and establishing well-defined agent-network interfaces for quick agent prototyping. NIKA comprises hundreds of curated network incidents, spanning five network scenarios, from data centers to ISP networks, and covers 54 representative network issues. Lastly, NIKA is modular and extensible by design, offering APIs to facilitate the integration of new network scenarios and failure cases. We evaluate state-of-the-art LLM agents on NIKA and find that while larger models succeed more often in detecting network issues, they still struggle to localize faults and identify root causes. NIKA is open-source and available to the community: https://github.com/sands-lab/nika.

==> assets/pseudocode.tex <==

\begin{figure}
  \begin{minipage}[t]{0.48\columnwidth}
  \begin{subfigure}[t]{\linewidth}
    \centering
    \begin{minted}[linenos=false, fontsize=\scriptsize]{python}
from nika import IncidentBase, IncidentInjectorTC,
                 ODFlowGenerator, Evaluator
class LinkBwThrottle(IncidentBase):
    name = "link_bandwidth_throttling"
    def __init__(self, net):
        self.net = net
        self.net.deploy()

    def inject_incident(self, dev, intf):
        self.dev = dev
        injector = IncidentInjectorTC(self.net)
        injector.inject_bw_limit(dev, intf, "1mbit")
        # Start traffic load
        od = ODFlowGenerator(self.net)
        od.set_src_dst(src="all", dst=dev)
        od.start_traffic(interval=20, speed="1mbps")

    def desc(self):
        return f"Latency increased in {self.net}."

    def eval(self, sub):
        Evaluator().eval(self, sub)
    \end{minted}
    \label{algo:problem}
    \caption{Defining an incident in \sysname.}
  \end{subfigure}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.48\columnwidth}
    \begin{subfigure}[t]{\linewidth}
        \centering
        \begin{minted}[linenos=false, fontsize=\scriptsize]{python}
from nika import exec
@mcp.tool()
async def exec_shell_dual(h1, cmd1, h2, cmd2):
    result1, result2 = await asyncio.gather(
        exec(h1, cmd1), exec(h2, cmd2))
    return {"host1": result1, "host2": result2}
        \end{minted}
        \caption{\sysname's MCP tool}
        \label{algo:mcp}
    \end{subfigure}
    
    \begin{subfigure}[t]{\linewidth}
        \centering
        \begin{minted}[linenos=false, fontsize=\scriptsize]{python}
from nika import LinkBwThrottle, DCClos
net = DCClos(size="s")
inc = LinkBwThrottle(net)
inc.inject_incident("host1", "eth0")
inc_desc = inc.desc()
        \end{minted}
        \caption{Instantiate a network incident}
        \label{algo:instance}
    \end{subfigure}

    \begin{subfigure}[t]{\linewidth}
        \centering
        \begin{minted}[linenos=false, fontsize=\scriptsize]{python}
from langchain.agents import create_agent
from nika import MCPServers
tools = MCPServers().tools
agent = create_agent(gpt-5, tools=tools)
submission = agent.run(inc_desc)
inc.eval(submission)
    \end{minted}
    \caption{Plugging in an agent.}
    \label{algo:agent}
    \end{subfigure}
\end{minipage}

  \caption{Code instrumentation examples.}
  \label{algo:nika-apis}
\end{figure}

==> notes.tex <==

\section{Introduction}\label{sec:intro}
\ac{if the paper is for conext we ca instead start with network-oriented intro}
Artificial Intelligence (AI) is shifting from human-oriented chat application to autonomous and interactive agentic systems with decision-making capabilities~\cite{}. Google has projected a 1 trillion USD market value for agentic AI by 2040~\cite{google-agentic-ai-report}.
% Agentic AI systems augment vanilla Language Models (LMs) with reasoning, tool use, and environment interaction.
This shift has accelerated the adoption of \llm in domains that require dynamic and context-aware operations, therefore expanding the horizon of AI applications to networking and systems.
\ac{fill gaps here..}
% In about one year, our community has moved from the very first investigations of \llm for selected networking use-cases (e.g., NetConfEval~\cite{wang2024netconfeval}, NetAssistant~\cite{wang2024netassistant}) to fully-fledged agentic systems used daily in production at hyperscalers such as Meta~\cite{wang2025intent} and Alibaba~\cite{bian} for their network management.
% Network vendors are also embracing the agentic AI trend~\cite{ericsson-ana}, and 
%Artificial Intelligence (AI) is expected to play a central role in enabling intent-based, adaptive, and autonomous behaviors across a broad range of networking domains, from emerging 6G architectures~\cite{..} to data center, optical and edge networks \cite{cui2025overview, zhou2024large}.

Network troubleshooting is a subset of network management:
given a network problem, network engineers undertake mechanical yet cumbersome steps to identify and remediate the issue~\cite{zoom2net,netseer,bufscope}.\ac{cite more} 
Common examples include probing the network to explain packet drops~\cite{netseer, bufscope} or refining the detection logic reasoning across heterogeneous telemetry \cite{} and diagnosis tools \ac{cite} -- \emph{e.g.}, 
request the collection of more fine-grained queue-length data to zoom into an ongoing incident~\cite{zoom2net}, enable debug-level diagnostics, etc.
The process is often manual, slow and error-prone, as it requires expert operators to reason across multiple dimensions. 

These characteristics make network troubleshooting a prominent candidate for agentic AI applications. 
Thanks to their ability to parse multimodal data and, more recently, engage in natural-language-driven reasoning~\cite{wang2024netconfeval, wang2024netassistant, netllmbench}, LMs hold a special promise for automate these tasks. We define \emph{\textbf{autonomous AI agents for network troubleshooting}} as \emph{systems that leverage \llm to autonomously interact with the network environment, collect and interpret telemetry data, and iteratively refine their diagnosis strategies to identify and resolve network issues with multi-turn  zero (or minimal) human intervention}.

\subsection{Limitations}
Recent work~\cite{wang2024netassistant,confucius,bian} shows that network operators already experiment with AI assistance to troubleshoot their networks. 
In parallel, the broader AI community is advancing agentic systems at fast pace.
% , to the point that agentic system can self-optimize their own prompts~\cite{} and architectures~\cite{}.
This evolution opens a rich design space for network troubleshooting agents, but our community currently lacks the benchmarks and platforms needed to explore and compare concrete designs in a principled way. Unfortunately, current systems such as NetAssistant~\cite{wang2024netassistant}, \textsc{BiAn}~\cite{} and Confucius~\cite{} are usually evaluated in bespoke, closed settings, with no publicly available datasets and limited disclosure of the evaluation scenarios.  In this section, we elaborate on 
the need for a standardized, reproducible, and open benchmarking platform, where to build and evaluate AI agents with low operational effort.

\smallskip
\smartparagraph{Design space: agents, tools, and context.}
Specifically, designers of AI agent applications must reason about dimensions such as:

\noindent \emph{Agent structure.} One can build a monolithic agent that handles end-to-end diagnosis, or decompose the task into multiple specialized agents (e.g., planning agent, active probers, telemetry experts, etc.).
  
\noindent \emph{Tool interfaces.} \ac{rephrase and make more clear typical challenges and questions for tools. The examples can go in background}Agents typically interact with the environment through tools that expose capabilities such as ping/traceroute, counter reads, INT queries, or SDN controller APIs~\cite{mcp}. The choice and granularity of these tools determine what actions the agent can take and which low-level details remain abstracted.
  
\noindent \emph{Context management and prompting.} Designers must decide which subset of topology, configuration, historical alerts, and previous actions is surfaced to the agent at each step, and how it is framed in prompts. This includes controlling thinking budget, structuring intermediate reasoning steps, and decide how and when to compact the context (i.e., previous observations and finidigs) to fit within model limits.

% These design questions are non-trivial even for experts in agentic AI, and they are opaque to many networking researchers. 
\noindent \underline{Takeaway:} 
A principled evaluation should compare different choices along these axes.

\smartparagraph{Limitations of current benchmarks.}
Today, no public benchmark targets this agent design space for network troubleshooting. NetConfEval~\cite{wang2024netconfeval}, for instance, focuses on configuration synthesis: given an intent and a partial network snapshot, an LLM generates device configurations that satisfy specified policies. NetConfEval is \emph{static}: each test case is a one-shot mapping from input text to configuration, with no closed-loop interaction, no evolving network state, and no notion of tools or multi-step reasoning. As a result, it cannot answer questions that are central to troubleshooting:
how well an agent sequences measurements and actions (e.g., which counters or probes to activate next); whether tool usage is efficient or redundant over time; how robustly an agent adapts its strategy when telemetry is noisy, delayed, or partially missing.
Furthermore, network troubleshooting tasks requires evaluation metrics that cannot be assessed by existing static benchmarks, such as time to resolution and impact on network performance during diagnosis.
% Therefore, we currently lack a dynamic benchmark that can exercise the interactive, decision-making behavior that defines troubleshooting agents.

\noindent \underline{Takeaway:} A benchmark of realistic network incidents is needed to evaluate agentic systems.

\smartparagraph{Lack of agent-network interfaces.}
Even if a corpus of annotated incident cases were available, it would still be insufficient for evaluating agentic systems. Network troubleshooting agents must operate in a \emph{live} environment where their actions (e.g., enabling INT, changing thresholds, issuing \texttt{ping}s) feed back into the network state and future observations. Production networks are unsuitable for this purpose due to safety, privacy, and reproducibility constraints. Existing emulators and testbeds~\cite{bonofiglio2018kathara,containerlab,mininet} solve part of the problem by providing controllable networks, but they stop short of offering:
\begin{enumerate*}[label=\emph{(\roman*)}]
  \item streamlined reproducibility of realistic incident scenarios;
  \item a unified agent–environment interface that exposes tools, telemetry, and evaluation hooks in a consistent way;
  \item orchestration of the end-to-end evaluation workflow, including performance evaluation and reasoning trajectory analysis.  
\end{enumerate*}

\noindent \underline{Takeaway:} \ac{make this takeaway stronger and more related to lack of something}
A plug-and-play platform to orchestrate end-to-end evaluation workflows is valuable to non-domain experts (e.g., AI engineers) to rapidly prototype their designs with low-effort learning curve, and even to domain-experts (e.g., network owners) to safely experiment with AI agents in controlled environments.


\section{Agentic AI}
\label{sec:agents}

\smartparagraph{From LMs to AI agents.}
Agentic AI systems augment a Language Model (LM) with reasoning capabilities and environment interactions. An agentic system embeds one or more LMs inside an \emph{agent} that iteratively observes the environment, reasons about intermediate states, and decides which action to take next~\cite{yao2023react,langgraph-workflows}. In this setting, the LM is one component in a closed loop that alternates between \emph{thought} (textual reasoning) and \emph{act} (issuing commands, invoking tools, or updating state) until a task-specific stopping condition is met.

\smartparagraph{Tools.}
A central mechanism in agentic AI is the notion of a \emph{tool}: a callable capability that lets the agent affect or query the outside world. Concretely, a tool is exposed as a structured API (e.g., ``ping from host A to host B'', ``read port counters on switch S'', ``query INT records for flow F'') with well-defined inputs and outputs. The LM does not execute these operations itself; instead, it decides \emph{when} to invoke which tool, with which arguments, and how to interpret the returned result. Frameworks such as MCP~\cite{mcp} standardize how such tools are described and surfaced to agents.

\smartparagraph{Multi-agent systems.}
Beyond a single agent, many applications adopt \emph{multi-agent systems} (MAS), where several agents with different roles collaborate on a shared task~\cite{du2023improving,li2025knowropesheuristicstrategy}. Each agent may use a different model, a different tool set, and hold a different state (i.e., memory). 
This decomposition allows agents to specialize in different sub-tasks and, more importantly, to manage context more effectively, by avoiding saturation of a shared context window.
% , and may only see a slice of the global context.
% For instance, one agent may specialize in triaging alerts, another in planning telemetry measurements, and a third in root-cause reasoning. Decomposing a complex task this way can reduce prompt complexity and and make behavior easier to validate, at the cost of designing coordination and information-passing among agents.




